The Perspectives of Non-Ideal Quantum Reference Frames

We define the perspective of any quantum reference frame (QRF) and construct reversible transformations between different perspectives. Our construction is based on two principles motivated operationally by the change from relative to absolute coordinates and leads to an incoherent group averaging approach with general symmetry group. Thereby, it extends the framework of [arXiv:2110.13199] from ideal QRFs, which generally require infinite resources like energy or angular momentum, to non-ideal QRFs, with only finite resources. We find that the perspective of a non-ideal QRF deviates significantly from that of an ideal QRF: Firstly, systems described relative to a non-ideal QRF appear superselected. Secondly, the structure of the perspective of a non-ideal QRF attests that successive relational operations on a system lead to back-reaction on this QRF.

==> figures_src/symbols.tex <==
\newcommand{\alice}[1][myyellow]{%
\begin{tikzpicture}[scale=2]%
    \fill[#1] (0,0) circle (0.06);%
    \fill[#1] (0.1,-0.3) -- (0.1,-0.17) arc(0:180:0.1) -- (-0.1,-0.3) -- cycle;%
    \node[white] at (0,-0.2) {\small$A$};%
\end{tikzpicture}%
}

\newcommand{\bob}[1][myyellow]{%
\begin{tikzpicture}[scale=2]%
    \fill[#1] (0,0) circle (0.06);%
    \fill[#1] (0.1,-0.3) -- (0.1,-0.17) arc(0:180:0.1) -- (-0.1,-0.3) -- cycle;%
    \node[white] at (0,-0.2) {\small$B$};%
\end{tikzpicture}%
}

\newcommand{\charlie}[1][myyellow]{%
\begin{tikzpicture}[scale=2]%
    \fill[#1] (0,0) circle (0.06);%
    \fill[#1] (0.1,-0.3) -- (0.1,-0.17) arc(0:180:0.1) -- (-0.1,-0.3) -- cycle;%
    \node[white] at (0,-0.2) {\small$C$};%
\end{tikzpicture}%
}

\newcommand{\atom}[1][]{%
    \begin{scope}[#1]%
    \foreach \x in {0,60,...,300}{%
        \fill[fill,thick] (\x:0.18) circle (0.18);%
    }%
    \foreach \x in {30,150,270}{%
        \draw[rotate=\x,thick] (0,0) ellipse (0.9 and 0.4);%
    }%
    \end{scope}%
}

\newcommand{\system}[1][myyellow]{%
\begin{tikzpicture}%
    \atom[#1,scale=0.5]%
    \node[white] at (0,0) {\small$S$};%
\end{tikzpicture}%
}

\newcommand{\gauge}[1][]{
    \begin{scope}[#1]
        \clip (-0.6,0) rectangle (0.6,0.6);
        \draw[thick] (0.5,0) arc[start angle=0,end angle=180,radius=0.5];
        \foreach \x in {20,40,...,160}{
            \draw[thick] (\x:0.5) -- (\x:0.4);
        }
        \node[fill,circle,inner sep=1pt] at (0,0) {};
        \draw[thick] (0,0) -- ++(50:0.4);
    \end{scope}
}

